ParaFuzz: An Interpretability-Driven Technique for Detecting Poisoned Samples in NLP

Backdoor attacks have emerged as a prominent threat to natural language processing (NLP) models, where the presence of specific triggers in the input can lead poisoned models to misclassify these inputs to predetermined target classes. Current detection mechanisms are limited by their inability to address more covert backdoor strategies, such as style-based attacks. In this work, we propose an innovative test-time poisoned sample detection framework that hinges on the interpretability of model predictions, grounded in the semantic meaning of inputs. We contend that triggers (e.g., infrequent words) are not supposed to fundamentally alter the underlying semantic meanings of poisoned samples as they want to stay stealthy. Based on this observation, we hypothesize that while the model's predictions for paraphrased clean samples should remain stable, predictions for poisoned samples should revert to their true labels upon the mutations applied to triggers during the paraphrasing process. We employ ChatGPT, a state-of-the-art large language model, as our paraphraser and formulate the trigger-removal task as a prompt engineering problem. We adopt fuzzing, a technique commonly used for unearthing software vulnerabilities, to discover optimal paraphrase prompts that can effectively eliminate triggers while concurrently maintaining input semantics. Experiments on 4 types of backdoor attacks, including the subtle style backdoors, and 4 distinct datasets demonstrate that our approach surpasses baseline methods, including STRIP, RAP, and ONION, in precision and recall.

==> rebuttal.tex <==
\clearpage
\newpage
We sincerely thank all the reviewers for the constructive comments. In the following, we first address a few common questions and then the individual reviewers' questions.
%\setcounter{section}{6}
\section{Usage of PICCOLO}
\label{sec:rb-piccolo}
%Q: What’s the relation between ParaFuzz and PICCOLO? Why not compare ParaFuzz with PICCOLO?
%If there is already a known poisoned set and even a known trigger, what is the contribution of ParaFuzz?
%Second, if we can successfully reverse what is the trigger pattern, why not just use some rule-based system to filter out samples with these identified patterns?

PICCOLO is a backdoor scanning tool aiming at detecting whether a language model is backdoored. It cannot reverse engineer exact triggers but optimizes a list of surrogate triggers that can induce ASR. As shown in Figure~\ref{fig:reversed}, the surrogate triggers reversed by PICCOLO usually differ completely from the ground-truth triggers. In contrast, \Tech{} has a different threat model and aims to identify poisoned samples. The surrogate triggers by PICCOLO cannot be directly used. Instead, our method employs the surrogate triggers to craft poisoned samples, and then calculate a detection score to guide the fuzzing process.

%\setcounter{figure}{8} 
\begin{figure}[h]
\centering
\includegraphics[width=0.99\linewidth]{Figs/table.pdf} 
\caption{The ground-truth triggers and PICCOLO-reversed triggers in the TrojAI dataset. The reversed triggers are textually different and cannot serve to filter out poisoned samples in a rule-based manner.}
\label{fig:reversed}
\end{figure}


%\setcounter{section}{7}
\section{Ablation study of meta prompts}
We evaluate the efficacy of individual meta prompts through an ablation study conducted on the first half of models from the TrojAI dataset. As depicted in Table~\ref{tab:abl-meta}, \Tech{} equipped with all three meta prompts generally performs the best, underscoring the effectiveness of each mutation strategy. Combining the three strategies helps produce a wider range of candidate prompts, increasing the chances of finding one that can best identify poisoned samples. 
The best prompts generated by \Tech{} and its versions without specific strategies are listed in Table 4 (in the Appendix) and Table~\ref{tab:abl-prompt}, respectively. Comprehensive comparisons suggest the prompts created by \Tech{} with all three meta prompts show a variety in words and structure.

In some cases, \Tech{} without one of the mutation strategies performs better. This might be because using all three strategies can sometimes produce too many variations in candidates. Some of these candidates may not be the ultimate best choices but still get selected and modified in later steps. Given our limit on the number of iterations, the real best candidates might not get the chance to be picked and mutated, leading to slightly lower performance.

%\setcounter{table}{4}
\begin{table}
  \caption{\Tech{} with all three meta prompts generally performs the best, suggesting the effectiveness of each mutation strategy.}
  \label{tab:abl-meta}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{crrrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{Model}  & \multicolumn{3}{c}{w/o keyword} & \multicolumn{3}{c}{w/o structure} & \multicolumn{3}{c}{w/o evolutionary} & \multicolumn{3}{c}{\Tech{}}              \\
    \cmidrule(r){2-4}\cmidrule(r){5-7}\cmidrule(r){8-10}\cmidrule(r){11-13}
    & Prec. (\%) & Recall (\%) & F1 (\%) & Prec. (\%) & Recall (\%) & F1 (\%) & Prec. (\%) & Recall (\%) & F1 (\%) & Prec. (\%) & Recall (\%) & F1 (\%) \\
    \midrule
12 & 93.9 & 89.9 & 91.8   & 94.8 & 86.7 & 90.6  & 97.4 & 79.8 & 87.7    & 98.8 & 87.8 & \textbf{93.0}\\
13 & 96.6 & 80.0 & 87.5  & 97.3&82.3 &89.2    & 95.9 & 79.4 & 86.9   & 93.2 & 86.3 & \textbf{89.6}\\
14 & 96.5 & 81.2 & 88.2  & 97.4&86.5 &91.6   & 93.7& 85.9 & 91.3    & 93.5&92.4&\textbf{92.9}\\
15 & 92.3 & 74.0 & 82.1  & 97.6& 84.9& 90.8   & 99.2 &87.0 & 92.7     & 96.9&87.0& 91.7\\
16 & 96.3 & 92.3 & 94.3  & 93.9&91.1 & 92.5   & 95.1 & 91.1 & 93.1   & 97.5&91.7&\textbf{94.5}\\
17 & 94.9 & 96.7 & 95.8   & 91.3& 88.9& 90.1   & 92.8 & 92.2 & 92.5    & 94.1&91.7&92.9\\
18 & 98.3 & 86.0 & 91.7  & 97.2& 88.0& 92.4   & 97.2 & 88.0 &  92.4   & 94.1&96.0&\textbf{95.0}\\
19 & 98.4 & 90.4 & 94.2  & 95.3& 92.4& 93.8   &  96.8&91.9  &94.3     & 95.7&90.9& 93.2\\
20 & 98.3 & 84.5 & 90.9   & 95.7& 77.7& 85.3   & 97.7 & 85.5 & 91.2  & 94.3&91.5&\textbf{92.9}\\
21 & 96.3 & 91.8 & 94.0  & 94.8&93.4 &94.1    & 97.3 & 93.4 & 95.3    & 
95.8&92.9&94.3\\
22 &91.9 & 80.3 & 85.7   & 96.0 &84.8 & 90.1   & 95.4 & 84.3 & 89.5      & 93.2&89.8&\textbf{91.5}\\ 
23 & 91.7 & 77.4 & 83.9 & 95.9& 81.8& 88.3   & 96.5 & 82.4 & 88.9    & 95.1&87.9&\textbf{91.4}\\
    \bottomrule
  \end{tabular}
  }
\end{table}


%\setcounter{table}{5}
\begin{table}
  \caption{The best prompts found during ablation study (case sensitive).}
  \label{tab:abl-prompt}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{clll}
    \toprule
    Model  & w/o keyword & w/o structure & w/o evolutionary    \\
    \midrule
12 & Soothe like a lullaby & Perform like a rockstar & Sigh tenderly resembling a draft\\
13 & sound like a rockstar & Unmute unlike a rockstar & Unalike a rock legend \\
14 & Buzz gently like a draft & Quiet as a rockstar & Quiet as a rockstar\\
15 & Resonate like a guitar & "Toneless, like an ordinary person" & Vocal as an ordinary individual\\
16 & Express yourself like a seasoned orator & Rock the stage like a superstar & Sigh like a gentle breeze\\
17 & Whisper like a breeze & Screaming like an anonymous fan & Flow like a river\\
18 & Compose like a master pianist & Quiet as a famous musician & Resemble a rockstar\\
19 & < > & Sound like a sound & Quiet as a rockstar\\
20 & Flow like a river & Resemble a sound & Resonate like a pitchfork \\
21 & Rumble like an earthquake & Hushed like a sound & Tune in harmony like an ensemble\\
22 & sound like a rockstar & Shout quietly & Compose melodies that resonate like a maestro\\
23 & sound like a rockstar & Loud unlike a silence & Ring like a bell\\
    \bottomrule
  \end{tabular}
  }
\end{table}

%\setcounter{section}{8}
\section{Adaptive attack}
An adaptive attack can involve the attacker mimicking ChatGPT's generation style as the trigger. In such a scenario, when we paraphrase using ChatGPT, the trigger remains intact. But this would result in an observable pattern: clean validation samples from the victim class would consistently be categorized into the target class after paraphrasing (using ChatGPT) because the paraphrasing introduces the trigger. Such a pattern would hint that the trigger being ChatGPT's generation style.

In this case, we can employ alternative Language Models (LLMs) in place of ChatGPT when running \Tech{} to still detect poisoned samples. It's also worth noting that identifying AI-generation style is difficult, and using it to poison a model presents significant challenges.


%\setcounter{section}{9}
\section{Alternatives of ChatGPT}
Our proposed technique is agnostic to any language model as the paraphraser and mutator. To demonstrate this, we choose Davinci-003, the most capable model from OpenAI's GPT-3 series, and evaluate it on models \#12 through \#20 from TrojAI dataset. As Table~\ref{tab:davinci} shows, \Tech{} integrated with davinci-003 still outperforms baselines on most models under evaluation.

%\setcounter{table}{6}
\begin{table}
  \caption{\Tech{} with Davinci-003 outperforms baselines on most models.\xz{cannot tell it outperforms, you may include the baseline results in the table}}
  \label{tab:davinci}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{ccccl}
    \toprule
    Model  & Precision (\%) & Recall (\%) & F1 (\%) & Best prompt    \\
    \midrule
12 & 91.9 & 91.0 & \textbf{91.4} & Discord like an experienced singer\\
13 & 90.1 & 78.2 & 83.7 &Whimper like a recording star\\
14 & 91.0 & 84.1& 87.4 &Utterances similar to an infant girl\\
15 & 85.3 & 80.0 & \textbf{82.6} &  Mute as a stone \\
16 & 88.0 & 91.1 & \textbf{89.5} & Talk with conviction like a politician boss \\
17 & 89.0 & 83.9 &  \textbf{86.4} & Resemble a superstar \\
18 & 94.0 & 78.0 & 85.2 & Write unlike a scientist \\
19 & 98.3 & 88.7 & \textbf{93.2} & Articulate like a debater \\
20 & 96.6 & 70.5 & \textbf{81.5} & Inexperienced as a music savant \\
    \bottomrule
  \end{tabular}
  }
\end{table}

%\setcounter{section}{10}
\section{Figures and tables for local response}
%\setcounter{figure}{9} 
\begin{figure}[h]
\centering
\includegraphics[width=0.99\linewidth]{Figs/coverage.png} 
\caption{The number of covered sentences w.r.t. iterations in style backdoor attack.}
\label{fig:coverage}
\end{figure}

%\setcounter{figure}{10} 
\begin{figure}[h]
\centering
\includegraphics[width=0.95\linewidth]{Figs/adversarial.png} 
\caption{Adversarial texts can be removed after paraphrasing.}
\label{fig:adv}
\end{figure}

%\setcounter{figure}{11} 
\begin{figure}[h]
\centering
\includegraphics[width=0.95\linewidth]{Figs/sophisticate.png} 
\caption{Manually devised sophisticated prompt fails to remove triggers from 7 out of 10 samples.}
\label{fig:sophisticate}
\end{figure}

\input{rebuttal1}
\input{rebuttal2}
\input{rebuttal3}
\input{rebuttal4}

==> rebuttal1.tex <==
\clearpage
%\setcounter{section}{11}
\section{Response to reviewer oHTu}
\subsection{Relation between PICCOLO and \Tech{}'s contribution} 
Please refer to global response.

%Q: How to configure ParaFuzz for prompts fuzzing for experiments in the paper and in general? Are they all the same or different configurations are needed for different NLP model and/or different input text lengths?
\subsection{Configuration of \Tech{}} 
The configuration of \Tech{} is the same for all NLP models, even with different input lengths. 

\subsection{Running time and iterations}
In experiments we set the maximum iterations to be 300 and the fuzzing process takes 143.88 minutes on average.

Take style backdoor attack as an example, Figure~\ref{fig:coverage} (see global response) illustrates the variation in coverage with respect to the number of iterations. The validation set contains 200 crafted poisoned sentences. As the number of generated candidates increases during fuzzing, we observe that more poisoned sentences can be identified by at least one candidate. Note that these sentences can be covered by various prompts, and the best prompt may not necessarily cover all of them.


\subsection{The prompts found by \Tech{}} 
The prompts found by \Tech{} are list in Table 4 in appendix.

%Q: Limitations were barely discussed in the paper. The proposed parafuzz has some limitations. ParaFuzz needs to know if the NLP model has changed its decision after the original text has been mutated. While for some NLP tasks it might be easy to check if the NLP decision changed, this is not always trivial.
\subsection{Limitations}
To identify the changes in the model's predictions, we simply call the model twice: one before the text is paraphrased, and the other after. By comparing the prediction labels from these two calls, we can easily determine if the model's decision has changed.
All ParaFuzz acquires from the model is the prediction labels. This is a minimal requirement compared to the baselines that need to manipulate the embedding layer or access the prediction probabilities.

==> rebuttal2.tex <==
\clearpage
%\setcounter{section}{12}
\section{Response to reviewer 7yjk}
\subsection{Alternative LLMs}
Please see the global response.

\subsection{Overhead}
In experiments, we set the maximum iterations to 300 for each model and the fuzzing process takes 143.88 minutes on average.

\subsection{ChatGPT as classifier}
We do not directly apply ChatGPT to classify, e.g., sentiment, because the poisoned model may have different classification standards than ChatGPT. For example, consider this comment with a positive label from TrojAI model \#36's training data, "Well, let me tell ya honey, this movie sure does paint a picture of what can happen when ya lose yer job in the auto industry. And don't even get me started on that CEO, what a real piece of work. But I gotta admit, it's quite the spectacle and I reckon anyone would get a kick outta watchin' this Michael Moore flick." It is classified, however, as negative by ChatGPT. Thus, we cannot simply replace the poisoned model with ChatGPT and neglect the standards.

\subsection{Adaptive attack}
Please see the global response.


==> rebuttal3.tex <==
\clearpage
%\setcounter{section}{13}
\section{Response to reviewer 6kxG}
%First, it can be a strong assumption to have some clean validation samples in the victim class. In addition, how to decide what is the victim class?
\subsection{Assumptions}
We adopt the same assumptions as the baselines. It's a standard practice for model users or owners to maintain a small set of clean samples to evaluate model performance. \Tech{} is designed to identify poisoned samples, implying that we are already aware of the model's contamination. The assumption of knowing the victim class is justified, as the detection of specific misclassifications would typically precede the recognition that the model has been poisoned.

\subsection{Rule-based system} As demonstrated in the global response section 7, since the reversed triggers by PICCOLO differ from the ground-truth triggers, it is impossible to employ a rule-based system to filter out poisoned samples. This is why we need \Tech{} to detect poisoned samples.

\subsection{Ablation study}
Please refer to the global response.

\subsection{Interpretability}
We define "model prediction interpretability" to mean that an NLP model's predictions for clean inputs should fundamentally depend on the semantic content of the sentences. If the model's prediction changes after paraphrasing, despite the semantics remaining unchanged, it suggests that the original prediction isn't based on semantics and therefore isn't interpretable. Such a change in prediction indicates the presence of a trigger in the original sentence before paraphrasing.

\subsection{Adversarial texts}
We evaluated the paraphrasing mechanism on adversarial textual inputs. Specifically, we selected three instances derived from the paper titled "Bad Characters: Imperceptible NLP Attacks", as shown in Figure~\ref{adv}. The inherent processing pipeline of ChatGPT automatically removes zero-width adversarial characters present in examples 2 and 3 even without paraphrasing. In the case of example 1, where the trigger is the "RIGHT-TO-LEFT OVERRIDE" character, we identify an optimized prompt, "sound like a poem", through fuzzing. This prompt enables successful restoration of the authentic numeral sequence "4321" post-paraphrasing.



==> rebuttal4.tex <==
\clearpage
%\setcounter{section}{14}
\section{Response to reviewer 4qgi}
\subsection{Hinge on ChatGPT}
Our technique is model-agnostic and can be generalized to any language models. For example, section 10 in the global response shows that alternative models can also achieve comparable performance.

\subsection{Ablation study}
See the global response. 

\subsection{Sophisticated prompts}
We have proceeded to evaluate the prompt you've suggested. 
We selected the first 10 sentences from the test set associated with the Hidden Killer attack, with the trigger being syntax structure S(SBAR)(,)(NP)(VP)(.)))).
As shown in Figure~\ref{fig:sophisticate}, the heuristics based sophisticated prompt fails to remove the trigger in 7/10 samples.
In fact, instead of devising heuristic prompts manually, we propose \Tech{} to make the process automatic by fuzzing, i.e., iteratively modifying the prompt candidates according to the reward.


\subsection{Sentence coverage and detection score}
True Positives quantify \textbf{how many} poisoned samples are accurately detected, while sentence coverage helps manage \textbf{which} poisoned samples are correctly identified. Inspired by code coverage in traditional fuzzing, we adopt sentence coverage as an auxiliary reward to retain candidates that accurately detect a challenging sample for the first time—a sample that previous candidates missed, even if their overall detection scores aren't the highest. Thus, we avoid the fuzzing process getting trapped in complex samples.

\subsection{Badnets in NLP}
Badnets is primarily known as a backdoor attack in the computer vision (CV) domain. However, the core idea behind Badnets can be generalized to natural language processing (NLP). 
In the CV context, Badnets typically involves embedding a specific pattern or "trigger" into images and labels them as the target class during training. When the poisoned model encounters samples with the trigger in the future, it predicts them as the target class.
For NLP, the same concept can be applied. Poisoned samples are generated by injecting a specific character/phrase/sentence (i.e., the trigger) into benign sentences and labeled as the target class. During training, the model learns to associate this trigger with the target prediction, regardless of the semantics of the sentences.

\subsection{Adaptive attack}
See the global response.

